Structure from Motion-based Motion Estimation and 3D Reconstruction of Unknown Shaped Space Debris

With the boost in the number of spacecraft launches in the current decades, the space debris problem is daily becoming significantly crucial. For sustainable space utilization, the continuous removal of space debris is the most severe problem for humanity. To maximize the reliability of the debris capture mission in orbit, accurate motion estimation of the target is essential. Space debris has lost its attitude and orbit control capabilities, and its shape is unknown due to the break. This paper proposes the Structure from Motion-based algorithm to perform unknown shaped space debris motion estimation with limited resources, where only 2D images are required as input. The method then outputs the reconstructed shape of the unknown object and the relative pose trajectory between the target and the camera simultaneously, which are exploited to estimate the target's motion. The method is quantitatively validated with the realistic image dataset generated by the microgravity experiment in a 2D air-floating testbed and 3D kinematic simulation.

==> macrosForEThesis.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%   macrosForEThesis.tex
%%   -------------------
%%
%%   Title: LaTeX macro file for the English Thesis
%%   
%%   
%%   Belief:
%%   1."Fig. 1: ~~~", "Table 1: ~~~" are for the figure and table citation.
%%   2. add the config to read the source code file (hello.c) and visualize it. 
%%
%%   Change Log:
%%   2020.11.26 Initial creation by Kentaro UNO
%%
%%   Contact:
%%   Please contact the author Kentaro UNO (unoken.astro@gmail.com) if
%%   you have a problem
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% useful command
\newcommand{\n}{\nonumber \\}
\newcommand{\p}{\partial}
\newcommand{\bs}[1]{\boldsymbol{#1}}
\newcommand{\II}{I\negthinspace I}
\newcommand{\III}{I\negthinspace I\negthinspace I}
\newcommand{\mbm}[1]{\mbox{\protect \boldmath $#1$}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  config for citation of figures, tables, and equations
%%%  to use English for all. 
%%%  2020.01.29 modified by Kentaro UNO
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% figure and table
\captionsetup{compatibility=false}
%
\renewcommand{\figurename}{Fig.~\hspace{-.2em}}   
\renewcommand{\tablename}{Table~\hspace{-.2em}}

\captionsetup[figure]{format=plain,labelformat=simple,labelsep=colon,font=small}
\captionsetup[table]{format=plain,labelformat=simple,labelsep=colon,font=small}

\newcommand{\bhline}[1]{\noalign{\hrule height #1}} % bhlineコマンドの設定

%%% citation command for figures, tables, and equations
\newcommand{\fig}[1]{Fig.~\ref{#1}}
\newcommand{\subfig}[2]{Fig.~\ref{#1}\subref{#2}}
\newcommand{\fign}[1]{\ref{#1}}
\newcommand{\tb}[1]{Table~\ref{#1}}
\newcommand{\tabn}[1]{\ref{#1}}
\newcommand{\eq}[1]{Eq.~(\ref{#1})}
\newcommand{\eqn}[1]{(\ref{#1})}

%%% citation command for chapters, sections, and appendixes
\newcommand{\chap}[1]{Chap.~\ref{#1}}
\newcommand{\sect}[1]{Sect.~\ref{#1}}
\newcommand{\subsect}[1]{Sect.~\ref{#1}}
\newcommand{\app}[1]{Appnd. ~\ref{#1}}

%%% visualize a figure and table in a row
\makeatletter
\newcommand{\figcaption}[1]{\def\@captype{figure}\caption{#1}}
\newcommand{\tblcaption}[1]{\def\@captype{table}\caption{#1}}
\makeatother

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  ソースコードの引用スタイルの設定
%%%  2020.01.24 added by Kentaro UNO
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{listings} %日本語のコメントアウトをする場合はjlistingが必要
%ここからソースコードの表示に関する設定
\definecolor{gray}{rgb}{0.9,0.9,0.9}
\lstset{
  backgroundcolor=\color{gray}, % choose the background color; you must add \usepackage{color} or \usepackage{xcolor}; should come as last argument
  basicstyle={\small\ttfamily}, % the style of the fonts that are used for the code
  identifierstyle={\small}, % main()の''main''等のスタイル
  commentstyle={\small\itshape}, %//comment 等のスタイル
  keywordstyle={\small}, % int mainの''int''等のスタイル
  ndkeywordstyle={\small},
  stringstyle={\small\ttfamily},  % string literal style -> % printf(''Hello'')の''''で囲まれた部分のスタイル
  %frame={tb},
  breaklines=true, % sets automatic line breaking
  columns=[l]{fullflexible},
  numbers=left, % where to put the line-numbers; possible values are (none, left, right)
  numberstyle={\scriptsize}, % the style that is used for the line-numbers
  stepnumber=1, % the step between two line-numbers. If it's 1, each line will be numbered
  numbersep=1zw, % 行数字とコードの間のマージン
  xrightmargin=0zw, % 表示個所の右側マージン
  xleftmargin=2zw,  % 表示個所の左側マージン
  rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
  showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
  showstringspaces=false,          % underline spaces within strings only
  showtabs=false,                  % show tabs within strings adding particular underscores
  lineskip=-0.5ex % codeの行間の設定
}

\def\epsgaiji#1{\leavevmode\kern-0.025zw\raise-.37zh\hbox{%
  \epsfile{file=#1,width=1.05zw}}\kern-0.025zw}
%\newcommand{\dfrac}[2]{\frac{\displaystyle{#1}}{\displaystyle{#2}}}
\newcommand{\MARU}[1]{{\ooalign{\hfil#1\/\hfil\crcr\raise.167ex\hbox{\mathhexbox20D}}}}

%%%
